A Sampling-based Framework for Hypothesis Testing on Large Attributed Graphs

Hypothesis testing is a statistical method used to draw conclusions about populations from sample data, typically represented in tables. With the prevalence of graph representations in real-life applications, hypothesis testing in graphs is gaining importance. In this work, we formalize node, edge, and path hypotheses in attributed graphs. We develop a sampling-based hypothesis testing framework, which can accommodate existing hypothesis-agnostic graph sampling methods. To achieve accurate and efficient sampling, we then propose a Path-Hypothesis-Aware SamplEr, PHASE, an m- dimensional random walk that accounts for the paths specified in a hypothesis. We further optimize its time efficiency and propose PHASEopt. Experiments on real datasets demonstrate the ability of our framework to leverage common graph sampling methods for hypothesis testing, and the superiority of hypothesis-aware sampling in terms of accuracy and time efficiency.

==> acknowledgement.tex <==
\section{Acknowledgement}
Reynold Cheng, Yun Wang, and Chrysanthi Kosyfaki were supported by the University of Hong Kong (Project 109000579), the HKU Outstanding Research Student Supervisor Award 2022-23, and the HKU Faculty Exchange Award 2024 (Engineering).

==> algorithms.tex <==
% \subsection{Hypothesis Aware Sampler}
% In this section, we delve into the hypothesis-aware design of PHASE and present its algorithm. We also introduce estimators for node, edge, and path hypotheses and demonstrate how PHASE facilitates the convergence of these estimators. Finally, to speed up the convergence, we introduce an optimized PHASE called Opt-PHASE.

% \subsection{PHASE Algorithm}
% % While many existing sampling methods can be adopted into our hypothesis testing framework, they often lack awareness of the underlying hypotheses, hence, resulting in varying hypothesis testing performance. Therefore, we have formulated three key objectives for the design of PHASE: (i) incorporating hypothesis awareness,(ii) achieving high accuracy in determining true and false outcomes of hypothesis testing, and (iii) ensuring fast execution. 

% The first objective in Section \ref{sec:problemStatement}, being aware of the hypothesis, is pivotal in establishing a path-hypothesis-aware sampling process. Also, the accuracy performance in the second objective highly depends on it. Thus, we delve into three types of sampling methods to understand how well they adapt to three hypothesis types. Node and edge samplers are designed for selecting nodes and edges directly from $\mathcal{G}$ but fall short in capturing paths. Consequently, they have slow convergence for path hypothesis as the number of relevant paths is limited. On the contrary, random walk-based samplers show effectiveness in preserving path information. 
% Therefore, we build the Path-Hypothesis-Aware SamplEr (PHASE) on \textit{FrontierS}, which provides wide uniform sampling of nodes in $\mathcal{G}$ and maintains the path-preserving property of random walks.
% % Its algorithm is illustrated in \ref{algo:FrontierS}. 
% % We assume the cost of randomly sampling a vertex to be $1$.

% \textbf{$m$-Dimensional Mechanism:} \textit{FrontierS} initiates $m$ seed nodes for random walks.
% % , as depicted in Algorithm ~\ref{algo:FrontierS} line 1. 
% This mechanism enhances the sampler's likelihood of selecting relevant nodes, edges, and paths from the original graph. Particularly, it is advantageous for selective hypotheses with strict modifiers, where hypothesis agnostic sampling methods often struggle to effectively sample relevant nodes, edges, or paths.

% \textbf{Random Walk Mechanism:} \textit{FrontierS} is a random walk based algorithm, which, when integrated with hypothesis awareness, can greatly benefit path hypotheses. \textit{FrontierS} selects a node from $m$ seeds based on degree-proportional probability and uniformly selects a neighbor.
% % , as illustrated in Algorithm ~\ref{algo:FrontierS} lines 4 and 6, respectively. 
% However, it shows slow convergence of hypothesis estimators due to the random selection of seed nodes and neighbors, resulting in missed targets.
% % The number of relevant nodes, edges, and paths will increase at a snail's pace as $B$ increases. 
% These two parts leave areas for us to incorporate hypothesis awareness. 
% % Specifically, by customizing the probability in line 4 and the transitional probability of random walk, we can bias the node and edge picking process towards the hypothesis.


% % \begin{algorithm}
% %     \caption{Frontier Sampler}
% %     \begin{algorithmic}[1]
% %         \Statex \textbf{Input:} $\mathcal{G}$, $B$
% %         \Statex \textbf{Output:} a sampled graph $\mathcal{G}_{\mathcal{S}}$
% %         \State Initialize $L=(v_1, v_2, \ldots, v_m)$ with $m$ randomly chosen nodes uniformly
% %         \State $\mathcal{V}_\mathcal{S}=\{\}$, $\mathcal{E}_\mathcal{S}=\{\}$
% %         \While{$B \geq m$}
% %             \State Select $v\in L$ with probability $\text{deg}(v)/\sum_{\forall u \in L}\text{deg}(u)$
% %             \State $N = v$'s neighbors
% %             \State Select $u \in N$ uniformly at random
% %             % \State $\mathcal{E}_\mathcal{S}$.add(\((v,u)\))
% %             \State $\mathcal{V}_\mathcal{S}$.update($v,u$)
% %             \State Replace $v$ by $u$
% %             \State $B=B-1$
% %         \EndWhile
% %         \State $\mathcal{G}_{\mathcal{S}} = \{\mathcal{V}_\mathcal{S},\mathcal{E}_\mathcal{S}\}$
% %     \end{algorithmic}
% %     \label{algo:FrontierS}
% % \end{algorithm} 


% The algorithm of PHASE is illustrated in Algorithm~\ref{algo:ours}. The inputs include $\mathcal{G}$, $B$, $\mathcal{P}$, and $H$. For a node hypothesis, $\mathcal{P}$ consists of a single node with length zero. For an edge hypothesis, the length of $\mathcal{P}$ is one. It initializes $m$ seeds in a list $L$ in Line 1. Each seed is assigned a weight in $L_w$ in Line 2. Lines 4-14 outline an iterative random walk process to select nodes until $B$ is reached. In the loop, the algorithm selects a node $v$ from $L$ with probability $L_w$ in Line 6. Subsequently, it selects one of $v$'s neighbors $u$ using a weighted selection process in Lines 7-9. After adding the selected nodes $u$ and $v$ to the sampled graph $\mathcal{V}_S$ in Line 10, the algorithm updates $L$ by replacing $v$ with $u$ and reduces the sampling budget in Lines 11 and 12, respectively. This iteration continues until $B \geq m$. The resulting sampled graph $\mathcal{G}_{\mathcal{S}}$ is the induced subgraph from $\mathcal{V}_S$.

% \begin{algorithm}
%     \caption{PHASE}
%     \begin{algorithmic}[1]
%         \Statex \textbf{Input:} $\mathcal{G} = (\mathcal{V, E})$, $B$,  $\mathcal{P}$, $H$
%         \Statex \textbf{Output:} a sampled graph $\mathcal{G_S} = (\mathcal{V_S, E_S})$
        
%         \State Initialize $L=(v_1, v_2, \ldots, v_m)$ with $m$ randomly chosen nodes uniformly
%         \State $L_w=\text{AssignWeight}(L,H)$
%         \State $\mathcal{V}_\mathcal{S}=\{\}$, $\mathcal{E}_\mathcal{S}=\{\}$
%         \While{$B \geq m$}
%             \State Normalize $L_w$
%             \State Select $v\in L$ with probability $L_w$
%             \State $N = v$'s neighbors
%             \State $N_w=\text{AssignWeight}(N,H)$
%             \State Select $u \in N$ with probability $N_w$ 
%             % \State $\mathcal{E}_\mathcal{S}$.add(\((v,u)\))
%             \State $\mathcal{V}_\mathcal{S}$.update($v,u$)
%             \State Replace $v$ by $u$ and update $L$ 
%             \State $B=B-1$
%         \EndWhile
%         \State $\mathcal{G}_{\mathcal{S}} = \{\mathcal{V}_\mathcal{S},\mathcal{E}_\mathcal{S}\}$
%     \end{algorithmic}
%     \label{algo:ours}
% \end{algorithm}

% The core components of PHASE are two weight functions, line 2 and 9 in Algorithm~\ref{algo:ours}. The former one determines the seed to start a random walk, while the latter one guides the random walk. Before introducing them, we denote two weights $w_1 \geq w_2 > 0$. We also denote $x_i$ as the nodes satisfying the $i$-th node condition on $\mathcal{P}$ and $y$ as the nodes which do not satisfying any node condition on $\mathcal{P}$. Equivalently, $x_i$ and $y$ represent different variable states in a random walk. For example, given a node hypothesis, there are only two states: $x_1$, and $y$.

% We use heuristics to design two weight functions. In line 2, $x_1$, representing the first node on $\mathcal{P}$ in three hypothesis types, is assigned a higher weight $w_1$ than all other nodes. In line 9, we adjust the transitional probability of random walk to bias the random walk process towards the nodes required by $H$.

% The transition probability matrices for node, edge, and path hypothesis are different as shown in Figure~\ref{fig:transition_prob} because they involve different states. A node hypothesis has two states: $x_1$ and $y$. Assuming the random walker is at a seed node $x_1$, $x_1$'s neighbors are either relevant ($x_1$) or irrelevant ($y$). We assign the higher weight $w_1$ to the transition to $x_1$ and the smaller weight $w_2$ to $y$, as shown in Figure~\ref{fig:transition_prob}a. Figure~\ref{fig:transition_prob}b shows an edge hypothesis has three states: $x_1$, $x_2$, and $y$. When the current state is $x_1$, we assign the higher weight $w_1$ to the transition to $x_2$. In other cases, we aim to pick the first node $x_1$ with a higher probability $w_1$.


% % Their transition probability matrices are shown in Figure~\ref{fig:transition_prob}a and ~\ref{fig:transition_prob}b, respectively. For a node hypothesis, assuming the random walker is at a seed node $x_1$, $x_1$'s neighbors are either relevant ($x_1$) or irrelevant ($y$). We assign the higher weight $w_1$ to the transition to $x_1$ and the smaller weight $w_2$ to $y$. In an edge hypothesis, $x_1$'s neighbors may include $x_1$, $x_2$, and $y$. When the current state is $x_1$, we assign the higher weight $w_1$ to the transition to $x_2$. 

% Besides differing in states, path hypotheses involve higher-order random walks rather than first-order ones. While the transition probability for a first-order random walk depends solely on the current state, that of a higher-order random walk depends on both the current and previous states. Figure~\ref{fig:transition_prob}c illustrates a part of the transition probability matrix for a second-order random walk in a path hypothesis of length three. Transitions between states are influenced by both the current and the last states. For instance, when the current state is $x_1$ and the previously visited state is $x_2$, the transition probability to $x_3$ is higher than to other states. Generally, a path hypothesis of length $l$ requires modeling by ($l-1$)-th order random walks.

% % , $x_1, x_2$ in edge hypothesis, $x_1, x_2, x_3$ in path hypothesis, and all irrelevant nodes as $y$. For node hypothesis, where we target to sample as many relevant nodes as possible through the sampling process, we have two types of 

% \begin{figure}
% \centering
% \begin{tikzpicture}[baseline={(current bounding box.south)}]
%   [column 1/.style={anchor=base},
%    column 2/.style={anchor=base},
%    column 3/.style={anchor=base}]
   
%   \matrix (left_matrix)
%    [nodes={minimum size=6mm,anchor=center}]
%   {
%     \node (left_matrix_1){}; & \node{$x_1$}; & \node {$y$}; \\ \hline
%     \node {$x_1$}; & \node[color=red]{$w_1$}; & \node {$w_2$}; \\
%     \node (left_matrix_7){$y$}; & \node[color=red]{$w_1$}; & \node {$w_2$}; \\
%   };
%     \draw (left_matrix_1.north east) -- (left_matrix_7.south east);
%     \node[below=0.9cm of left_matrix,font=\small] {(a)};
    
%     \matrix (mid_matrix) [right=0.1cm of left_matrix,nodes={minimum size=6mm,anchor=center}]
%   {
%    \node (mid_matrix_1){}; & \node{$x_1$}; & \node{$x_2$} ; & \node {$y$}; \\ \hline
%     \node {$x_1$}; & \node{$w_2$}; & \node[color=red]{$w_1$}; & \node {$w_2$}; \\
%      \node {$x_2$}; & \node[color=red]{$w_1$}; & \node{$w_2$}; & \node {$w_2$}; \\
%     \node (mid_matrix_7){$y$}; & \node[color=red]{$w_1$}; & \node{$w_2$}; & \node {$w_2$}; \\
%   };
%   \draw (mid_matrix_1.north east) -- (mid_matrix_7.south east);
%   \node[below=0.6cm of mid_matrix,font=\small] {(b)};
  
%   \matrix (right_matrix) [right=0.1cm of mid_matrix,nodes={minimum size=6mm,anchor=center}]
%   {
%    \node (right_matrix_1)[minimum width=8mm]{}; & \node{$x_1$}; & \node{$x_2$}; & \node{$x_3$}; & \node {$y$}; \\ \hline
%     \node [minimum width=8mm]{$x_1, x_1$}; & \node{$w_2$}; & \node[color=red]{$w_1$}; & \node{$w_2$}; & \node {$w_2$}; \\
%     \node [minimum width=8mm]{$x_1, x_2$}; & \node{$w_2$}; & \node{$w_2$}; & \node[color=red]{$w_1$}; & \node {$w_2$}; \\
%     \node [minimum width=8mm]{$x_1, x_3$}; & \node[color=red]{$w_1$}; & \node{$w_2$}; & \node{$w_2$}; & \node {$w_2$}; \\
%     \node (right_matrix_7)[minimum width=8mm]{$x_1, y$}; & \node[color=red]{$w_1$}; & \node{$w_2$}; & \node{$w_2$}; & \node {$w_2$}; \\
%   };
%   \draw (right_matrix_1.north east) -- (right_matrix_7.south east);
%   \node[below=-0.4cm of right_matrix,font=\small] {$\vdots$};
%   \node[below=0.3cm of right_matrix,font=\small] {(c)};
% \end{tikzpicture}
% \caption{The transition probability matrices for node hypothesis (a), edge hypothesis (b), and path hypothesis (c)}
% \label{fig:transition_prob}
% \end{figure}

% \subsection{Opt-PHASE Algorithm}
% To achieve the third objective, we implement two optimizations as shown in Algorithm ~\ref{algo:Opt-PHASE} to replace line 7 in Algorithm ~\ref{algo:ours}. Firstly, in a densely connected AHIN, the computation of neighbor weights in step 8 of Algorithm \ref{algo:ours} can be time-consuming due to the potentially large number of neighbors. To mitigate this, we randomly sample a subset of $\max\{|N|,n\}$ neighbors as candidates for selection, thereby reducing computation overhead. In the experiment, we set $n=30$. Secondly, to speed up the effective sampling, we adopt a non-backtracking approach by avoiding the selection of visited nodes during the sampling process\cite{DBLP:conf/sigmetrics/LeeXE12}. This strategy prioritize the selection of relevant nodes, edges, or paths, hence improving the efficiency and effectiveness of PHASE.


% \begin{algorithm}
%     \caption{Opt-PHASE}
%     \begin{algorithmic}[1]
%         \Statex \textbf{Input:} $\mathcal{G} = (\mathcal{V, E})$, $B$,  $\mathcal{P}$, $H$
%         \Statex \textbf{Output:} a sampled graph $\mathcal{G_S} = (\mathcal{V_S, E_S})$
%         \State $N' = v\text{'s neighbors other than the previous node}$  (Opt 2)
%         % \State $N = \max\{len(N),n\}$ neighbors as $N$, where $n=30$ (Opt 1)
%         \State $N = \text{max}\{ |N|, n \} \text{ nodes from } N$ (Opt 1)
%     \end{algorithmic}
%     \label{algo:Opt-PHASE}
% \end{algorithm} 


% \subsection{Convergence of Estimators}
% By Lemma 5.1 from~\cite{DBLP:conf/imc/RibeiroT10}, \textit{FrontierS} is equivalent to the sampling process of a \textit{SRW} over $\mathcal{G}^m=(\mathcal{V}^m,\mathcal{E}_m)$, where $\mathcal{G}^m$ is the $m$-th Cartesian power of $\mathcal{G}$ and
% \[\mathcal{V}^m=\{(v_1,\ldots,v_m)|v_1 \in \mathcal{V} \wedge \dots \wedge v_m \in \mathcal{V}\}\]
% is the $m$-th Cartesian power of $\mathcal{V}$.
% $\forall \boldsymbol{u,v} \in \mathcal{V}^m$,
% $(\boldsymbol{u,v}) \in \mathcal{E}_m$ if there exists $i$ such that $(u_i,v_i)\in \mathcal{E}$ and for all $j \neq i$, $u_j = v_j$. Given $\mathcal{G}$ is directed, connected, and non-bipartite graph $\mathcal{G}$, in steady state, sampled edges of \textit{FrontierS} form a stationary sequence and satisfy the Strong Law of Large Number (SLLN).

% \begin{theorem}[SLLN]
%     For any function $f$, where \\ $\sum_{(u,v)\in \mathcal{E}}|f(u,v)|<\infty$,
%     \[\lim_{B\to\infty} \frac{1}{B}\sum^{B}_{i=1}f(u_i,v_i) \to \frac{1}{|E|}\sum_{\forall (u,v)\in\mathcal{E}}f(u,v)\]
%     almost surely, i.e. the event occurs with probability one.
% \label{thm:SLLN}
% \end{theorem}

% For a node or edge hypothesis, PHASE adjusts the transition probability used in \textit{FrontierS}. But it ensures that the resulting random walk maintains both irreducibility and aperiodicity, thereby preserving stationarity and adhering to the SLLN. A path hypothesis with length $l$ involves a $(l-1)$-th order random walk, which can be by a \textit{SRW} over $\mathcal{G}^{l-1}=(\mathcal{V}^{l-1},\mathcal{E}_{l-1})$. Consequently, for a path hypothesis of length $l$, PHASE's random walk can be viewed as a \textit{SRW} over $\mathcal{G}^{l-1+m}=(\mathcal{V}^{l-1+m},\mathcal{E}_{l-1+m})$. As a result, the SLLN applies based on the same reasoning. Since the stationary distribution of the \textit{NBRW} remains the same as that of the \textit{SRW}, Opt-PHASE also follows the SLLN.

% By Theorem~\ref{thm:SLLN}, estimators can be constructed for node, edge, and path hypotheses. An \textbf{estimator} is a function applied to a sequence of observations to estimate an unknown population parameter, which is the primary subject of the node, edge, or path hypothesis. Here, we focus on scenarios where $\text{agg}$ represents an average function. Estimators for other aggregation functions, such as maximum and minimum, can be derived in a similar manner. 

% For a node hypothesis $\textit{avg}(t_i[attr_j]|M_{t_i})$, its primary subject is $t_i[attr_j]$. Let $\mathcal{V}^* \subseteq \mathcal{V}$ be all relevant nodes satisfying $M_{t_i}$. The mean value of the node hypothesis, $\theta_{node}$, is 
% \begin{equation}
%  \theta_{node} = \frac{1}{|\mathcal{V}^*|}\sum_{\forall (u,v) \in \mathcal{E}} \frac{S(v)}{deg(v)}
%  \label{eq:1}
% \end{equation}
% where $S(v) = \phi(v)[a_j] \times \mathbbm{1}_{M_{t_i}\subseteq \mathcal{L}_{\phi(v)}}$, which returns the attribute value $\phi(v)[a_j]$ if $v$ satisfies $M_{t_i}$ and 0 otherwise. By replacing $\mathcal{E}$ with a sequence of sampled edges $B$, the estimator for $\theta_{node}$ is
% \begin{equation}
% \hat{\theta}_{node} = \frac{1}{|B \cap \mathcal{V}^*|}\sum_{i=1}^{B} \frac{S(v_i)}{deg(v_i)}
% \label{eq:2}
% \end{equation}
% By Theorem~\ref{thm:SLLN}, we have 
% \begin{equation}
% \lim_{B\to\infty} \frac{1}{|B \cap \mathcal{V}^*|}\sum_{i=1}^{B} \frac{S(v_i)}{deg(v_i)} \to \frac{1}{|\mathcal{V}^*|}\sum_{\forall (u,v) \in \mathcal{E}} \frac{S(v)}{deg(v)}
% \label{eq:3}
% \end{equation}
% almost surely. This implies that $\hat{\theta}_{node}$ is an asymptotically unbiased estimator of $\theta_{node}$.

% For a path hypothesis $\text{avg}(f_{\mathcal{P}}| M_{t_i}, \forall t_i \text{ on } \mathcal{P})$, its primary subject is $f_{\mathcal{P}}$. Let $\mathcal{P}^*$ be all relevant paths such that each node on it satisfies the corresponding modifier, and $\mathcal{P_G}$ be all paths with the same length as $\mathcal{P}$ in $\mathcal{G}$. The mean value of the path hypothesis, $\theta_{path}$, is 
% \begin{equation}
%  \theta_{path} = \frac{1}{|\mathcal{P}^*|}\sum_{\forall \mathcal{P} \in \mathcal{P_G}} T(\mathcal{P})
%  \label{eq:4}
% \end{equation}
% where $T(\mathcal{P}) = f_{\mathcal{P}} \times \mathbbm{1}_{M_{t_i}\subseteq \mathcal{L}_{\phi(t_i)} \forall t_i \text{ on } \mathcal{P}} $. Replacing $\mathcal{G}$ with the sampled graph $\mathcal{G_S}$, the estimator for $\theta_{path}$ is
% \begin{equation}
% \hat{\theta}_{path} = \frac{1}{|\mathcal{P}^*\cap\mathcal{P_{G_S}}|}\sum_{\forall \mathcal{P} \in \mathcal{P_{G_S}}} T(\mathcal{P})
% \label{eq:5}
% \end{equation}
% When $B$ goes to infinity, $\mathcal{G_S}$ converges to $\mathcal{G}$. By Theorem~\ref{thm:SLLN}, we have 
% \begin{equation}
% \lim_{B\to\infty} \frac{1}{|\mathcal{P}^*\cap\mathcal{P_{G_S}}|}\sum_{\forall \mathcal{P} \in \mathcal{P_{G_S}}} T(\mathcal{P}) \to \frac{1}{|\mathcal{P}^*|}\sum_{\forall \mathcal{P} \in \mathcal{P_G}} T(\mathcal{P})
% \label{eq:6}
% \end{equation}
% almost surely. Hence, $\hat{\theta}_{path}$ is an asymptotically unbiased estimator of $\theta_{path}$. A path hypothesis becomes a edge when $l=1$. Based on the same argument, one can obtain the estimator for an edge hypothesis and prove its convergence.

